3D-aware Blending with Generative NeRFs

Image blending aims to combine multiple images seamlessly. It remains challenging for existing 2D-based methods, especially when input images are misaligned due to differences in 3D camera poses and object shapes. To tackle these issues, we propose a 3D-aware blending method using generative Neural Radiance Fields (NeRF), including two key components: 3D-aware alignment and 3D-aware blending. For 3D-aware alignment, we first estimate the camera pose of the reference image with respect to generative NeRFs and then perform 3D local alignment for each part. To further leverage 3D information of the generative NeRF, we propose 3D-aware blending that directly blends images on the NeRF's latent representation space, rather than raw pixel space. Collectively, our method outperforms existing 2D baselines, as validated by extensive quantitative and qualitative evaluations with FFHQ and AFHQ-Cat.

==> supp_sections/3_2_ours_poisson.tex <==



\section{Ours with Poisson Blending}
\label{sec:ours_poisson}
\begin{comment}
\paragraph{Ablation study with an extra user study.}
\ifdefined\ARXIV
   In Tables \ref{tbl:baseline_edit_celeba} and \ref{tbl:baseline_edit_afhq}, 
\else
   In Tables 1 and 2 of the paper, 
\fi
we report the combination of our method and Poisson blending. It shows Poisson blending further enhances the performance of our method in all automatic metrics: KID, m$L_2$, and LPIPS$_m$. In the realism score of human perception, ours with Poisson Blending outperforms other baselines, as shown in 
\ifdefined\ARXIV
   \reftbl{baseline_userstudy}.
\else
   Table 3 of the paper.
\fi

We conduct an extra user study to measure how far Poisson blending affects the realism score of human perception in our blending method. Tables~\ref{tbl:suppUserCelebA} and \ref{tbl:suppUserAFHQ} show the comparison with baselines in photorealism, and we use exactly the same experimental setting and test images as 
\ifdefined\ARXIV
   \reftbl{baseline_userstudy}.
\else
   Table 3 in the paper.
\fi
Combining our 3D-aware blending method with Poisson blending shows improvement in most cases.
%, as shown in \reftbl{suppUserCelebA} and \reftbl{suppUserAFHQ}. 
\end{comment}
% Please note that our method solely outperforms other baselines without Poisson blending. 
% Additional qualitative comparison can be seen in \reffig{suppfigOurs_w_wo_PB}. 






\paragraph{Implementation details.} We perform Poisson blending between the original image and the blended image generated by our 3D-aware blending method. 
Our blending method is modified in two ways. 1) In the initial blending stage, we only preserve the area around the border of the mask instead of all parts of the original image, as we can directly use the original image in the Poisson blending stage. This makes blending easier and reduces the number of iterations from 200 to 100, resulting in improved faithfulness scores (m$L_2$ and LPIPS$_m$) as shown in 
\ifdefined\ARXIV
   Tables \ref{tbl:baseline_edit_celeba} and \ref{tbl:baseline_edit_afhq}.
\else
   Tables 1 and 2 of the paper. 
\fi 
2) Instead of using the latent code of the original image $\w{ori}$ as the initial value of $\w{edit}$, we use the latent code of the reference image $\w{ref}$. This allows us to instantly reflect the identity of the reference image and only optimize $\w{edit}$ to reconstruct a small region of the original image.
Note that we apply Poisson blending to our method in 
\ifdefined\ARXIV
Figures~\ref{fig:motivation},~\ref{fig:ablationalign},~\ref{fig:disentangle},~\ref{fig:suppfigCompareCelebA} and \ref{fig:suppfigCompareAFHQ} and Tables~\ref{tbl:baseline_edit_celeba} and \ref{tbl:baseline_edit_afhq}.
\else
Figures 1, 5, and 8 in the main paper.
% and Figures ~\ref{fig:suppfigCompareCelebA} and \ref{fig:suppfigCompareAFHQ}.
% Tables~\ref{tbl:baseline_edit_celeba} and \ref{tbl:baseline_edit_afhq}.
\fi

\suppfigPoissonBaseline


\paragraph{Poisson blending with baselines.}
We combine Poisson blending with our method to achieve near-perfect background preservation. This is an optional choice, and our method \emph{without} Poisson blending has already outperformed all the baselines, as shown in 
\ifdefined\ARXIV
   Tables \ref{tbl:userstudyCelebA} and \ref{tbl:userstudyAFHQ}.
\else
   Tables 3 and 4 of the paper.
\fi 
Besides, combining Poisson blending with each baseline does not have meaningful benefits, as shown in \reffig{poisson_baseline}. 


